Do We Need All the Synthetic Data? Targeted Image Augmentation via Diffusion Models

Synthetically augmenting training datasets with diffusion models has become an effective strategy for improving the generalization of image classifiers. However, existing approaches typically increase dataset size by 10-30x and struggle to ensure generation diversity, leading to substantial computational overhead. In this work, we introduce TADA (TArgeted Diffusion Augmentation), a principled framework that selectively augments examples that are not learned early in training using faithful synthetic images that preserve semantic features while varying noise. We show that augmenting only this targeted subset consistently outperforms augmenting the entire dataset. Through theoretical analysis on a two-layer CNN, we prove that TADA improves generalization by promoting homogeneity in feature learning speed without amplifying noise. Extensive experiments demonstrate that by augmenting only 30-40% of the training data, TADA improves generalization by up to 2.8% across diverse architectures including ResNet, ViT, ConvNeXt, and Swin Transformer on CIFAR-10/100, TinyImageNet, and ImageNet, using optimizers such as SGD and SAM. Notably, TADA combined with SGD outperforms the state-of-the-art optimizer SAM on CIFAR-100 and TinyImageNet. Furthermore, TADA shows promising improvements on object detection benchmarks, demonstrating its applicability beyond image classification. Our code is available at https://github.com/BigML-CS-UCLA/TADA.

==> ICLR_2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> contents/Archived.tex <==
% \begin{table}[t]
% \caption{Test classification error of ResNet18 on CIFAR10, CIFAR100 and TinyImageNet.}
% \label{tab:dateset}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Method & CIFAR10 & CIFAR100 & Tiny ImageNet \\
% \midrule
% ERM    & 5.28 & 22.98 & 33.66 \\
% ERM+aus & 5.00 & 22.59 & 33.70 \\
% ERM+ta    & 4.32 & 21.05 & 30.84 \\
% ERM+aus+ta    & 4.13 & \textbf{20.33} & 31.5 \\
% ERM+syn     & 4.83 & 21.69 & 32.9 \\
% ERM+syn-all      & 4.66 & 21.21 & 33.14 \\
% ERM+syn+ta      & \textbf{3.68} & \underline{20.55}& \textbf{29.74} \\\midrule
% SAM   & 4.21 & 21.07 & 32.9 \\
% SAM+aus   & 4.01 & 21.16 & 32.52 \\
% SAM+ta   & 4.01 & 19.64 & 29.58 \\
% SAM+aus+ta   & 3.57 & \textbf{18.92} & 29.82 \\
% SAM+syn   & 3.69 & 20.17 & 30.58 \\
% SAM+syn-all   & 3.93 & 19.73 & 30.10 \\
% SAM+syn+ta   & \textbf{3.49} & \underline{19.03} & \textbf{28.14} \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[t]
% \caption{Test classification error of ResNet18 on CIFAR10, CIFAR100 and TinyImageNet.}
% \label{tab:dateset}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \scalebox{0.9}{
% \begin{tabular}{lcccr}
% \toprule
% Method & CIFAR10 & CIFAR100 & Tiny ImageNet \\
% \midrule
% ERM    & 5.07 $\pm$ 0.04 & 23.09 $\pm$ 0.25 & 34.04 $\pm$ 0.30 \\
% ERM+aus & 4.79 $\pm$ 0.05 & 22.34 $\pm$ 0.16 & 33.73 $\pm$ 0.07 \\
% ERM+ta    & 4.25 $\pm$ 0.07 & 21.10 $\pm$ 0.21 & 31.25 $\pm$ 0.17 \\
% ERM+aus+ta    & 4.00 $\pm$ 0.10 & \underline{20.47 $\pm$ 0.11} & 31.19 $\pm$ 0.28 \\
% ERM+syn     & 4.68 $\pm$ 0.02 & 21.13 $\pm$ 0.19 & 32.9 \\
% ERM+syn-all      & 4.78 $\pm$ 0.04 & 21.31 $\pm$ 0.07 & 33.14 \\
% ERM+syn+ta      & \textbf{3.81 $\pm$ 0.10} & \textbf{19.83 $\pm$ 0.17}& \textbf{29.74} \\\midrule
% SAM   & 4.23 $\pm$ 0.08 & 21.48 $\pm$ 0.27 & 32.45 $\pm$ 0.37 \\
% SAM+aus   & 4.04 $\pm$ 0.06 & 20.95 $\pm$ 0.05 & 31.83 $\pm$ 0.28 \\
% SAM+ta   & 4.06 $\pm$ 0.08 & 19.63 $\pm$ 0.07 & 29.93 $\pm$ 0.19 \\
% SAM+aus+ta   & 3.49 $\pm$ 0.09 & \textbf{18.94 $\pm$ 0.03} & 29.21 $\pm$ 0.18 \\
% SAM+syn   & 3.84 $\pm$ 0.11 & 19.78 $\pm$ 0.03 & 30.58 \\
% SAM+syn-all   & 3.99 $\pm$ 0.05 & 20.01 $\pm$ 0.05 & 30.10 \\
% SAM+syn+ta   & \textbf{3.56 $\pm$ 0.05} & 18.21 $\pm$ 0.10 & \textbf{28.14} \\
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[t]
% \caption{Test classification error of VGG19, DenseNet121 and ViT-S on CIFAR10.}
% \label{tab:architecture}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Architecture & VGG19 & DenseNet121 & ViT-S \\
% \midrule
% ERM    & 6.87 & 10.42 & 19.77 \\
% ERM+aus & 6.22 & 10.05 & 19.29 \\
% ERM+ta    & 6.15 & 9.65 & 19.62 \\
% ERM+aus+ta    & 5.37 & \textbf{8.58} & 18.19 \\
% ERM+syn     & 6.20 & 10.32 & 18.01 \\
% ERM+syn-all      & 5.82 & 9.92 & \textbf{17.78} \\
% ERM+syn+ta      & \textbf{5.06} & \underline{9.08} & \underline{17.79} \\\midrule
% SAM   & 5.79 & 9.4 & 19.64 \\
% SAM+aus   & 5.57 & 8.76 & 18.68 \\
% SAM+ta   & 5.67 & 9.53 & 20.41 \\
% SAM+aus+ta   & 4.88 & 8.38 & 18.76 \\
% SAM+syn   & 5.17 & \underline{8.28} & 17.66 \\
% SAM+syn-all   & 4.96 & \textbf{8.03} & \textbf{17.09} \\
% SAM+syn+ta   & 5.44 & 8.62 & \underline{17.48} \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[t]
% \caption{Test classification error of VGG19, DenseNet121 and ViT-S on CIFAR10.}
% \label{tab:architecture}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \scalebox{0.9}{
% \begin{tabular}{lcccr}
% \toprule
% Architecture & VGG19 & DenseNet121 & ViT-S \\
% \midrule
% ERM    & 6.68 $\pm$ 0.15 & 10.43 $\pm$ 0.02 & 20.27 $\pm$ 0.40 \\
% ERM+aus & 6.34 $\pm$ 0.09 & 10.00 $\pm$ 0.04 & 19.57 $\pm$ 0.24 \\
% ERM+ta    & 5.88 $\pm$ 0.20 & 9.45 $\pm$ 0.15 & 19.68 $\pm$ 0.27 \\
% ERM+aus+ta    & 5.43 $\pm$ 0.09 & \underline{8.76 $\pm$ 0.42} & 18.06 $\pm$ 0.37 \\
% ERM+syn     & 6.02 $\pm$ 0.02 & 9.56 $\pm$ 0.09 & 17.96 $\pm$ 0.06 \\
% ERM+syn-all      & 6.10 $\pm$ 0.05 & 9.85 $\pm$ 0.08 & 18.04 $\pm$ 0.16 \\
% ERM+syn+ta      & \textbf{5.25} $\pm$ 0.06 & \textbf{8.70 $\pm$ 0.06} & 17.32 $\pm$ 0.22 \\\midrule
% SAM   & 5.80 $\pm$ 0.07 & 9.40 $\pm$ 0.05 & 20.11 $\pm$ 0.33 \\
% SAM+aus   & 5.54 $\pm$ 0.03 & 8.89 $\pm$ 0.06 & 18.99 $\pm$ 0.22 \\
% SAM+ta   & 5.74 $\pm$ 0.06 & 9.49 $\pm$ 0.11 & 20.37 $\pm$ 0.12 \\
% SAM+aus+ta   & 5.11 $\pm$ 0.17 & 8.46 $\pm$ 0.15 & 17.89 $\pm$ 0.62 \\
% SAM+syn   & 5.12 $\pm$ 0.04 & 8.54 $\pm$ 0.10 & 17.65 $\pm$ 0.12 \\
% SAM+syn-all   & 5.26 $\pm$ 0.06 & 8.64 $\pm$ 0.10 & 17.92 $\pm$ 0.19 \\
% SAM+syn+ta   & 5.09 $\pm$ 0.03 & 8.51 $\pm$ 0.12 & 17.50 $\pm$ 0.02 \\
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[t]
% \caption{Training ResNet18 on CIFAR10 with different upsampling factor (k). \TODO{Try more seeds for generation.} \jh{Fig 4 have been updated too.}}
% \label{tab:up_factor}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lccc}
% \toprule
% k & Generation (Cifar10) & Upsampling (Cifar10) & Generation (Cifar100)\\
% \midrule
% 2   & 4.73 $\pm$ 0.19 & 4.79 $\pm$ 0.05 & 21.13 \\
% 3   & 4.72 $\pm$ 0.09 & 5.01 $\pm$ 0.16 & 21.27 \\
% 4   & 4.52 $\pm$ 0.12 & 5.04 $\pm$ 0.13 & 20.26 \\
% 5   & 4.45 $\pm$ 0.05 & 4.98 $\pm$ 0.09 & 20.00 \\
% 6   & 4.55 & 5.10
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{figures/vary_uf_same_seed.pdf}}
% \caption{\textbf{Ablation study of training ResNet18 on CIFAR10.} We used the standard training settings while varying upsampling factor with the same seed and same steps.}
% \label{fig:diff_uf_same_seed}
% \end{center}
% \vskip -0.2in
% \end{figure}

% Table \ref{tab:dateset} illustrates the performance of models trained with SGD and SAM using original, USEFUL and our method. We can see that our method effectively reduce test classification error of both SGD and SAM than USEFUL method.

% \begin{table}[t]
% \caption{Test classification error of ResNet18 on CIFAR10, CIFAR100, and Tiny-ImageNet. }
% \label{tab:dateset}
% % \vskip 0.15in
% \vspace{-1mm}
% \begin{center}
% \begin{small}
% \begin{sc}
% \scalebox{0.9}{
% \begin{tabular}{llccc}
% \toprule
% Optimizer & Aug dataset & CIFAR10 & CIFAR100 & Tiny-ImageNet \\
% \midrule
% SGD & Original & 5.07 $\pm$ 0.04 & 23.09 $\pm$ 0.25 & 34.04 $\pm$ 0.30 \\
% & \useful & 4.79 $\pm$ 0.05 & 22.34 $\pm$ 0.16 & 33.73 $\pm$ 0.07 \\
% & \textbf{Ours} & \textbf{4.42 $\pm$ 0.03} & \textbf{20.60 $\pm$ 0.27} & \textbf{31.55 $\pm$ 0.24} \\
% \midrule
% SAM & Original & 4.23 $\pm$ 0.08 & 21.48 $\pm$ 0.27 & 32.45 $\pm$ 0.37 \\
% & \useful & 4.04 $\pm$ 0.06 & 20.95 $\pm$ 0.05 & 31.83 $\pm$ 0.28 \\
% & \textbf{Ours} & \textbf{3.72 $\pm$ 0.10} & \textbf{18.84 $\pm$ 0.22} & \textbf{29.04 $\pm$ 0.04} \\
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[t]
% \caption{Test classification error of ResNet18 on CIFAR10, CIFAR100 and TinyImageNet.}
% \label{tab:dateset}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \scalebox{0.9}{
% \begin{tabular}{lcccr}
% \toprule
% Method & CIFAR10 & CIFAR100 & Tiny ImageNet \\
% \midrule
% ERM    & 5.07 $\pm$ 0.04 & 23.09 $\pm$ 0.25 & 34.04 $\pm$ 0.30 \\
% ERM+aus & 4.79 $\pm$ 0.05 & 22.34 $\pm$ 0.16 & 33.73 $\pm$ 0.07 \\
% ERM+ta    & 4.25 $\pm$ 0.07 & 21.10 $\pm$ 0.21 & 31.25 $\pm$ 0.17 \\
% ERM+aus+ta    & 4.00 $\pm$ 0.10 & \underline{20.47 $\pm$ 0.11} & 31.19 $\pm$ 0.28 \\
% ERM+syn     & 4.42 $\pm$ 0.03 & 20.60 $\pm$ 0.27 & 31.55 $\pm$ 0.24 \\
% ERM+syn-all      & 4.78 $\pm$ 0.04 & 21.31 $\pm$ 0.07 & 32.89 $\pm$ 0.24 \\
% ERM+syn+ta      & \textbf{3.25 $\pm$ 0.04} & \textbf{18.43 $\pm$ 0.18}& \textbf{28.72 $\pm$ 0.48} \\\midrule
% SAM   & 4.23 $\pm$ 0.08 & 21.48 $\pm$ 0.27 & 32.45 $\pm$ 0.37 \\
% SAM+aus   & 4.04 $\pm$ 0.06 & 20.95 $\pm$ 0.05 & 31.83 $\pm$ 0.28 \\
% SAM+ta   & 4.06 $\pm$ 0.08 & 19.63 $\pm$ 0.07 & 29.93 $\pm$ 0.19 \\
% SAM+aus+ta   & 3.49 $\pm$ 0.09 & 18.94 $\pm$ 0.03 & 29.21 $\pm$ 0.18 \\
% SAM+syn   & 3.72 $\pm$ 0.10 & 18.84 $\pm$ 0.22 & 29.04 $\pm$ 0.04 \\
% SAM+syn-all   & 3.99 $\pm$ 0.05 & 20.01 $\pm$ 0.05 & 30.32 $\pm$ 0.40 \\
% SAM+syn+ta   & \textbf{3.08 $\pm$ 0.08} & \textbf{17.11 $\pm$ 0.11} & \textbf{27.05 $\pm$ 0.24} \\
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[!t]
% \caption{Test classification error of VGG19, DenseNet121, and ViT-S on CIFAR10.}
% \label{tab:architecture}
% % \vskip 0.15in
% \vspace{-1mm}
% \begin{center}
% \begin{small}
% \begin{sc}
% \scalebox{0.9}{
% \begin{tabular}{llccc}
% \toprule
% Optimizer & Aug dataset & VGG19 & DenseNet121 & ViT-S \\
% \midrule
% SGD & Original & 6.68 $\pm$ 0.15 & 10.43 $\pm$ 0.02 & 20.27 $\pm$ 0.40 \\
% & \useful & 6.34 $\pm$ 0.09 & 10.00 $\pm$ 0.04 & 19.57 $\pm$ 0.24 \\
% & \textbf{Ours} & \textbf{6.02 $\pm$ 0.02} & \textbf{9.56 $\pm$ 0.09} & \textbf{17.96 $\pm$ 0.06} \\
% \midrule
% SAM & Original & 5.80 $\pm$ 0.07 & 9.40 $\pm$ 0.05 & 20.11 $\pm$ 0.33 \\
% & \useful & 5.54 $\pm$ 0.03 & 8.89 $\pm$ 0.06 & 18.99 $\pm$ 0.22 \\
% & \textbf{Ours} & \textbf{5.12 $\pm$ 0.04} & \textbf{8.54 $\pm$ 0.10} & \textbf{17.65 $\pm$ 0.12} \\
% \bottomrule
% \end{tabular}
% }
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{figure}[!t]
% % \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{figures/vary_uf_syn.pdf}}
% \caption{The effect of the upsampling factor $k$ on the performance of training ResNet18 on the augmented CIFAR10 dataset produced by our method and \useful. Red points indicate the optimal choice of $k$ for each method.}
% \label{fig:vary_uf_syn}
% \end{center}
% \vskip -0.2in
% \end{figure}


% \begin{figure}[ht]
% % \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{figures/denoising_strategy.pdf}}
% \caption{Comparison between synthetic CIFAR10 images generated from random noises and real images when training ResNet18 on the augmented set. For reference, we include the performance of the original training set.}
% \label{fig:denoising_strategy}
% \end{center}
% \vskip -0.2in
% \end{figure}

% \begin{table}[t]
% \caption{FID and test classification error of ResNet18 on CIFAR10 with different steps of generation.}
% \label{tab:fid}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Steps & FID & ERM & SAM \\
% \midrule
% 0(original images)   &       & 5.00 & 4.01 \\
% 10                   & 5.36  & 5.15 & 4.03 \\
% 20                   & 6.86  & 5.01 & 3.92 \\
% 30                   & 7.48  & 5.01 & 3.79 \\
% 40                   & 8.52  & 4.91 & 3.92 \\
% 50                   & 10.67 & \underline{4.87} & \textbf{3.69} \\
% 60                   & 13.25 & 4.98 & \underline{3.72} \\
% 70                   & 17.46 & 4.91 & 3.84 \\
% 80                   & 24.27 & \textbf{4.83} & 3.98 \\
% 90                   & 34.69 & 5.17 & 3.86 \\
% 100                  & 47.35 & 4.99 & 4.28 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}

% \begin{table}[t!]
%     \vskip -0.1in
%     \centering
%     \caption{Test classification error of pre-trained ResNet18 on Flowers-102, Aircraft, and Stanford Cars datasets. Synthetic images are generated using the DiffuseMix~\citep{islam2024diffusemix} pipeline \ba{?}}.
%     \label{tab:transfer_learning}
%     \vskip -0.1in
%     \begin{tabular}{c|c|c|c}
%         \toprule
%         Method & Flowers-102 & Aircraft & Stanford Cars \\
%         \midrule
%         Original & 8.55 $\pm$ 0.19 & 26.02 $\pm$ 0.27 & 15.45 $\pm$ 0.02 \\
%         DiffuseMix & 8.92 $\pm$ 0.15 & 25.65 $\pm$ 0.20 & 15.19 $\pm$ 0.06 \\
%         Ours & \textbf{8.08} $\pm$ \textbf{0.16} & \textbf{25.12} $\pm$ \textbf{0.35} & \textbf{14.96} $\pm$ \textbf{0.07} \\
%     \end{tabular}
%     \vskip -0.2in
% \end{table}

% \begin{table}[!t]
%     \centering
%     \caption{Test classification error of ConvNeXt-T and Swin-T on CIFAR-10 using SGD with $k = 2$.}
%     \label{tab:sota_arch}
%     \vskip 0.15in
%     \begin{tabular}{c|c|c|c}
%         \toprule
%         Method & ConvNeXt-T & Swin-T \\
%         \midrule
%         Original & 37.33 $\pm$ 3.12 & 16.10 $\pm$ 0.19 \\
%         \useful & 34.16 $\pm$ 2.47 & 14.93 $\pm$ 0.07 \\
%         Ours & \textbf{27.40} $\pm$ \textbf{1.99} & \textbf{14.57} $\pm$ \textbf{0.10} \\
%     \end{tabular}
% \end{table}

% \begin{table}[t!]
%     \vskip -0.1in
%     \centering
%     \caption{(left) Test classification error of ConvNeXt-T and Swin-T on CIFAR-10 using SGD with $k = 2$. (right) Test classification error of pre-trained ResNet18 on Flowers-102, Aircraft, and Stanford Cars datasets.}
%     \label{tab:combined_results}
%     \vskip -0.1in
%     \begin{subtable}[t]{0.4\textwidth}
%         \centering
%         % \caption{Test classification error of ConvNeXt-T and Swin-T on CIFAR-10 using SGD with $k = 2$.}
%         % \caption{}
%         \label{tab:sota_arch}
%         \scalebox{0.8}{
%         \begin{tabular}{c|c|c}
%             \toprule
%             Method & ConvNeXt-T & Swin-T \\
%             \midrule
%             Original & 37.33 $\pm$ 3.12 & 16.10 $\pm$ 0.19 \\
%             \useful & 34.16 $\pm$ 2.47 & 14.93 $\pm$ 0.07 \\
%             Ours & \textbf{27.40} $\pm$ \textbf{1.99} & \textbf{14.57} $\pm$ \textbf{0.10} \\
%             \bottomrule
%         \end{tabular}
%         }
%     \end{subtable}
%     \hfill
%     \begin{subtable}[t]{0.55\textwidth}
%         \centering
%         % \caption{Test classification error of pre-trained ResNet18 on Flowers-102, Aircraft, and Stanford Cars datasets.}
%         % \caption{}
%         \label{tab:transfer_learning}
%         \scalebox{0.8}{
%         \begin{tabular}{c|c|c|c}
%             \toprule
%             Method & Flowers-102 & Aircraft & Stanford Cars \\
%             \midrule
%             Original & 8.55 $\pm$ 0.19 & 26.02 $\pm$ 0.27 & 15.45 $\pm$ 0.02 \\
%             DiffuseMix & 8.92 $\pm$ 0.15 & 25.65 $\pm$ 0.20 & 15.19 $\pm$ 0.06 \\
%             Ours & \textbf{8.08} $\pm$ \textbf{0.16} & \textbf{25.12} $\pm$ \textbf{0.35} & \textbf{14.96} $\pm$ \textbf{0.07} \\
%             \bottomrule
%         \end{tabular}
%         }
%     \end{subtable}
%     % \vskip -0.2in
% \end{table}

==> contents/Diffusion_process.tex <==

\subsection{Generating Faithful Synthetic Images via Diffusion Models} \label{subsec:diffusion}


Finally, we discuss generating \textit{faithful} images for the slow-learnable part of the data. From Theorem \ref{thm:noise_overfitting} we know that while the noise in the synthetic data can be larger than that of the original data, it should be small enough to yield a similar feature learning behavior to SAM. %\ba{Leo check this} \Leo{Yes, this is true. It should definitely }

% \textbf{Diffusion Models.} 
Synthetic image generation with diffusion models \citep{pmlr-v37-sohl-dickstein15,ho_denoising_2020,pmlr-v139-nichol21a,10.1145/3626235} %are a class of probabilistic generative models that gradually destroy data by injecting noise, then learn to reverse this process for sample generation.
% generate synthetic images by adding noise to the images and  then learn to reverse this process.
involves a forward process to iteratively add noise to the images, followed by a reverse process to learn to denoise the images.
Specifically, the forward process progressively adds noise to the data $x_0$ over $T$ steps, with each step modeled as a Gaussian transition: $q(\mathbf{x}_t | \mathbf{x}_{t-1}) = \mathcal{N}(\mathbf{x}_t; \sqrt{1-\beta_t} \mathbf{x}_{t-1}, \beta_t \mathbf{I})$, where $\beta_t$ controls the noise added at each step. The reverse process inverts the forward process, learns to denoise the data, with the goal of recovering the original data $x_0$ from a noisy sample $x_T$: $ p_\theta(\mathbf{x}_{t-1} | \mathbf{x}_t) = \mathcal{N}(\mathbf{x}_{t-1}; \mu_\theta(\mathbf{x}_t, t), \Sigma_\theta(\mathbf{x}_t, t)) $, where mean $ \mu_\theta $ is conditioned on the sample at the previous time step and variance $\Sigma_\theta $ follows a fixed schedule.\looseness=-1


% In the process of generating images using diffusion models, we selected an open-source text-to-image model, GLIDE \citep{nichol2022glidephotorealisticimagegeneration}, as our baseline for image generation. 
% We employed the USEFUL method proposed by \citep{nguyen2024data} to identify examples that benefit the most from synthetic data augmentation. This approach allowed us to effectively select relevant examples that could be enhanced through the addition of synthetic images.

% To generate faithful images, we utilized a real guidance strategy \citep{he_is_2023} that integrates synthetic images into the training dataset. Specifically, while using the class name (e.g., "a photo of a dog") as the text prompt, we also incorporated the original real samples as guidance. In this process, the real samples—after being slightly modified with added noise—replace the random noise at the initial stage of image generation, guiding the diffusion process. 
% This approach enables us to produce synthetic images that are similar, yet distinct, from the original examples. By doing so, we not only diversify the dataset but also maintain the authenticity of the training data, ensuring that the synthetic images remain faithful rather than drastically different from the real ones.

To ensure generating images that are faithful to real data, we use the real images as guidance to generate synthetic images. 
Specifically, while using the class name (e.g., ``a photo of a dog'') as the text prompt, we also incorporated the original real samples as guidance. 
% In this process, the real samples—after being slightly modified with added noise—replaces the random noise at the initial stage of image generation, guiding the diffusion process.
% This technique enables produce synthetic images that are similar, yet distinct, from the original examples, and has been successfully used for synthetic image generation for few-shot learning \citep{he_is_2023}. 
% Formally, in a normal text-to-image generation process, a pure noisy image $x_T \sim \mathcal{N}(0, I)$ is sampled first as the initialization of the reverse path. 
More formally, instead of sampling a a pure noisy image $x_T \sim \mathcal{N}(0, I)$ as the initialization of the reverse path,  
%In our case, 
we add noise to a reference (real) image $x_0^{ref}$ such that the noise level corresponds to a certain time-step $t_*$. %I.e., $x_{t_*}^{ref}=$
%Then, rather than sampling from time-step $T$, we initialize the noisy latent variable as $x_{t_*}^{ref}$ and 
Then we begin denoising from time-step $t_*$, using an open-source text-to-image model, e.g. GLIDE \citep{nichol2021glide}, to iteratively predict a less noisy image $x_{t-1} (t = T, T - 1, \cdots, 1)$ using the given text prompt $l$ and the noisy latent image $x_t$ as inputs.
% This effectively increases the action consistency for examples in the cluster with higher gradient norm.
This technique enables produce synthetic images that are similar, yet distinct, from the original examples, and has been successfully used for synthetic image generation for few-shot learning \citep{he_is_2023}. 
%that our
% The middle row shows synthetic images of slow-learnable samples generated using GLIDE described in Section~\ref{subsec:diffusion}. These 
% synthetic examples preserve key visual content (features) such as object shape, structure, and spatial arrangement while introducing subtle variations in texture or color (noise). 
% For instance, an image of a bird in the second row is reproduced with the same layout and pose, but with different color for the neck part.
% an image of a person riding a horse (column "horse") is reproduced with the same layout and pose, but with slightly lighter tones for the head and body. 
%
% This approach enables us to produce synthetic images that are similar, yet distinct, from the original examples. By doing so, we not only diversify the dataset but also maintain the authenticity of the training data, ensuring that the synthetic images remain faithful rather than drastically different from the real ones.
Our pseudocode is illustrated in Appendix~\ref{app:pseudocode} Alg. \ref{alg:Method}. \looseness=-1
%Our algorithm is similar to \useful~except that in Step 3, we replace the real images by synthetic images generated as above. 
% \ba{somewhere we should say our method is similar to useful or add a pseudocode}



